On the complexity of range searching among curves

Modern tracking technology has made the collection of large numbers of densely sampled trajectories of moving objects widely available. We consider a fundamental problem encountered when analysing such data: Given $n$ polygonal curves $S$ in $\mathbb{R}^d$, preprocess $S$ into a data structure that answers queries with a query curve $q$ and radius $\rho$ for the curves of $S$ that have \Frechet distance at most $\rho$ to $q$. We initiate a comprehensive analysis of the space/query-time trade-off for this data structuring problem. Our lower bounds imply that any data structure in the pointer model model that achieves $Q(n) + O(k)$ query time, where $k$ is the output size, has to use roughly $\Omega\left((n/Q(n))^2\right)$ space in the worst case, even if queries are mere points (for the discrete \Frechet distance) or line segments (for the continuous \Frechet distance). More importantly, we show that more complex queries and input curves lead to additional logarithmic factors in the lower bound. Roughly speaking, the number of logarithmic factors added is linear in the number of edges added to the query and input curve complexity. This means that the space/query time trade-off worsens by an exponential factor of input and query complexity. This behaviour addresses an open question in the range searching literature: whether it is possible to avoid the additional logarithmic factors in the space and query time of a multilevel partition tree. We answer this question negatively. On the positive side, we show we can build data structures for the \Frechet distance by using semialgebraic range searching. Our solution for the discrete \Frechet distance is in line with the lower bound, as the number of levels in the data structure is $O(t)$, where $t$ denotes the maximal number of vertices of a curve. For the continuous \Frechet distance, the number of levels increases to $O(t^2)$.

==> ddlb.tex <==
\section{The Lower Bound in Higher Dimensions}
In this section, we generalize the lower bound for the multilevel stabbing problem to $\R^d$.
Many of the ingredients of the previous lower bound can be carried to higher dimensions, however, there are
some crucial theorems and lemmas where we need non-trivial replacement. 
Furthermore, these replacements come with much higher degree of technical difficulty.
One major difference is that for our lower bound in 2D, we can cleanly separate an ``orthogonal subproblem''
(represented by Lemma~\ref{lem:orthc} and the fact that we only need to care about the volume
of axis-aligned boxes created by the parametric points).
In higher dimensions, this is no longer the case.

The beginning of our proof is very similar to the previous proof however.
As before, we define the space $\Q = \Q_1 \times \Q_2 \times \dots \Q_t$ where each $\Q_i$ is
the unit cube $[0,1]^d$ in $\R^d$.
One face of these unit cubes is designated to be the {\em top} face.
$\Q$ now represents the set of all possible queries
and an input $t$-slab $\bs$ is represented by picking $t$ independent slabs, one slab $\ts{i}$ in $\Q_i$
for each $1 \le i \le t$.
$\Q$ is the unit hypercube in the  $((d-1)t)$-dimensional space and thus $\vol_{(d-1)t}(\Q) = 1$.
\begin{observation}\label{ob:volproductdd}
  For any $t$-slab $\bs$, $\vol_{2t}(\bs) = \vol_2(\ts{1})\cdot\vol_2(\ts{2})\dots \cdot \vol_2(\ts{t})$. 
\end{observation}
Again similar to the previous proof, we would like to build 
$r$ different input sets $\S_1, \dots, \S_r$, for a parameter $r$, such that:
(i) each $\S_i$ contains $\Theta(n/r)$ $t$-slabs,
(ii) the slabs defined in each $\Q_i$ will be parallel, and
(iii) for any two $t$-slabs  $\bs_1, \bs_2 \in \S_i$, we have
$\vol_{2t}(\bs_1\cap \bs_2) = 0$.


\subsection{Defining Parameters of $\S_i$}
To define each $\S_i$, we need more parameters. 
We will use a $t$ point $\phi(\S_i) = (\alpha^{(1)}_i, \alpha^{(2)}_i, \dots, \alpha^{(t)}_i)$ where
each $\alpha_i^{(j)}$ is a point on the top face of $\Q_j$. 
We will also use $t-1$ integral
parameters $w^{(1)}_i, w^{(2)}_i, \dots, w^{(t-1)}_i$.  
We call these the {\em defining parameters of $\S_i$}.  
The point $\phi(\S_i)\in \R^{(d-1)t}$ is called the parametric point of $\S_i$
and the tuple $\C(\S_i) = (w^{(1)}_i, w^{(2)}_i, \dots, w^{(t-1)}_i)$ is defined as the {\em color} of $\S_i$.
Similarly, every slab $\bs \in \S_i$ is said to have the same parametric point and color.
In other words, we define $\phi(\bs) = \phi(\S_i)$ and $\C(\bs) = \C(\S_i)$ for every $\bs \in \S_i$.
Each point $\alpha^{(i)}$ is going to define the direction of the slabs in $\Q_i$.
Also, we will use a global parameter $R$ when constructing all the $\S_i$'s and we
define $w^{(t)}_i = \log_R(n/r) - \sum_{j=1}^{t-1}w^{(j)}_i$ and $W^{(j)}_i = R^{-w^{(j)}_i}$, for $1 \le j \le t$
and $W^{(1)}_i, W^{(2)}_i, \dots, W^{(t)}_i$ are going
to be the thickness of the slabs in $\S_i$.
Finally, for a set of $\beta$ sets $\S_1, \dots, \S_\beta$ where
$\phi(\S_i) = (\alpha^{(1)}_i, \alpha^{(2)}_i, \dots, \alpha^{(t)}_i)$, we define a {\em parametric region} 
which is defined as $\preg(\S_1, \dots, \S_\beta) = \conv(\alpha_1^{(1)}, \alpha_2^{(1)}, \dots, \alpha_\beta^{(1)}) \times
\times \dots \times \conv(\alpha_1^{(t)}, \alpha_2^{(t)}, \dots, \alpha_\beta^{(t)})$ and 
a {\em parametric volume}  that defined as $\pvol(\S_1, \dots, \S_\beta) = \vol_{(d-1)t}(\preg(\S_1, \dots, \S_\beta))$.
In other words, to obtain the parametric region of $\S_1, \dots, \S_\beta$, we look at the set of points placed at the 
top face of each $\Q_i$, and then form the Cartesian product of these regions. 
The parametric volume is the ($(d-1)t$-dimensional) volume of the parametric region. 

\begin{observation}\label{ob:ddwidthprod}
    \[ \prod_{1\le j \le t} W^{(j)}_i= \left( \prod_{1\le j \le t-1} W^{(j)}_i \right) W^{(t)}_i= R^{-(\sum_{j=1}^{t-1}w^{(j)}_i)  - w^{(t)}_i}= \frac rn.\]
\end{observation}


These defining parameters are used to define the slabs in the following way.
Consider $\S_i$ with its defining parameters $\phi(\S_i)$ and $\C(\S_i)$.
For every square $\Q_j$, $1 \le j \le t$, we will define a set, $\S_{i,j}$, 
of ordinary slabs in the following way.  
We consider the point $\alpha^{(j)})_i$ as a point on the top face of $\Q_i$.
We connect the origin to the point $\alpha^{(j)})_i$ and 
We define the set $\S_{i,j}$ of slabs as the set of disjoint and parallel slabs that are perpendicular to the line
connecting the origin to the point $\alpha^{(j)})_i$ such that they tile the entire $\Q_i$ and the width 
of each slab is $W^{(j)}_i$.
The set $\S_i$ is defined as the Cartesian product of the sets
$S_{i,1}\times \ldots \times S_{i,t}$.

\begin{figure}
\centering
\includegraphics{figs/ddhyperslabs}
\caption{Each ${\mathcal S}_i$ is defined as the Cartesian product of $t$ sets
of $d$-dimensional slabs which each tile the unit square.  Any two $t$-slabs from
the same set ${\mathcal S}_i$ have empty common intersection.}
\end{figure}


Thus, for each $\S_i$, it remains to pick $\phi(\S_i)$ and $\C(\S_i)$.
To get our lower bound, this needs to be done very carefully and it involves various technical steps. 

\subsection{Picking the Set of Colors}
The set of colors are picked according to Lemmas~\ref{lem:easygood} and~\ref{lem:hardgood}.
However, this just creates the set of colors $\C_g$ that we can use to color the parametric points
defining the sets $\S_i$. 
To decide which parametric points to pick and which color to assign to them still needs an intricate design
that we do in the next subsection.

\subsection{Picking the Parametric Points}
To pick the set of parametric points, we begin by the following results.
We first start by result that is a generalization of a previous bound. 
\begin{lemma}\cite{Chazelle.simplex.RR.LB}\label{lem:parallel}
    Consider a unit cube $\Q$ in $\R^d$ and let $f$ be its top face.
	Consider $d$ points $p_1, \dots, p_d \in f$ and let $s_i$ be a slab with
    width $w_i$ that is perpendicular to the line connecting the origin to $p_i$. 
    Define $V=\bigcap_{1\le i \le d} S_{i}$. 
    We have $\vol_d(V) =  O\left( \frac{\prod_{i=1}^d w_i}{ \vol_{d-1}\conv(p_1, \dots, p_d)} \right)$
    in which $\conv(.)$ denotes the convex hull of a set of points. 
\end{lemma}

The above lemmas implies a direct connection between a set of slabs having small intersection with the volume of the
convex hull the points the define the slabs. 
Unfortunately, this takes us to a very difficult unresolved but related question:
for a fixed value $k\ge 3$, over all placements of $n$ points in the unit square in $\R^2$, what is the maximum value of the 
area of the convex hull of $k$ points?
This problem, known as Heilbronn's triangle problem for when $k=3$, has been a major bottleneck is obtaining tight lower bounds for
problems such as simplex range reporting (see~\cite{Chazelle.simplex.RR.LB,a12} for more details on this
bottleneck).     
In particular, if one can show that for a constant value of $k$, it is possible to place $n$ points such that
the convex hull of every $k$ points has area at least $\Omega(1/n)$, then we can obtain tight lower bounds for simplex
range reporting in 3D. 
As discussed, this is a very difficult problem to resolve and thus the existing approaches to obtain simplex range reporting
lower bounds is to somehow circumvent this open problem by aiming for a weaker claim
(we relax the requirement that $k$ be a constant and that the volume be $\Omega(1/n)$).
Furthermore, in our case, we need to be able to deal with the Cartesian products of $t$ unit squares rather than
just one unit square. 
The next lemma is the main tool that we borrow
from~\cite{Chazelle.LB.JAMath89}.

\begin{lemma}\cite{Chazelle.LB.JAMath89}\label{lem:convex}
	Consider the unit hypercube in $d$ dimensions in which $d$ is a constant.
	For any real value $0 < \rho < 1$, there exists a set $\B_\rho$ of $1/\rho^{O(1)}$ 
	convex shapes inside the unit hypercube such that each shape in 
	$\B_\rho$ has volume $O(\rho)$ and for any convex shape $A$ of volume at
	most $\rho$, there exists a convex shape in $\B_\rho$ that completely contains $A$.
\end{lemma}

Let $\beta$, $\rho$ and $\rho_c$ be three global parameters to be decided later. 
For now, we will assume that $\rho$ will be set such that $\rho = o(1/(c_0^tr))$ and 
$\rho_c = o( |\C_g| / (c_0^tr))$ for a constant $c_0$.
Consider the unit squares $\Q_1, \dots \Q_t$.
At the top face of each $\Q_i$, we build the following set of convex shapes.
For every value of $\rho_{i,j} = 2^{-j}, 0 \le j \le \log n$, we create a set $\B_{i,j}$
according to the above theorem with $\rho_{i,j}$ as the real-valued parameter. 
For every indices $j_1, j_2, \dots, j_t$ such that
$ \rho\le \rho_{i,j_1}  \rho_{i,j_2}  \dots  \rho_{i,j_t}  \le 2^t \rho$, we build the Cartesian product 
of the shapes in $\B_{i,j}$, that is, 
$\B_{i,j_1}\times \B_{i,j_2}\times \dots \times \B_{i,j_t}$.
Next, for every indices $j_1, j_2, \dots, j_t$ such that
$ \rho_c \le \rho_{i,j_1}  \rho_{i,j_2}  \dots  \rho_{i,j_t}  \le 2^t \rho_c$, we build the Cartesian product 
of the shapes in $\B_{i,j}$, that is, 
$\B_{i,j_1}\times \B_{i,j_2}\times \dots \times \B_{i,j_t}$.
Let $\B_c$ be the set of all such regions built.
By above lemma, we have that $|\B| = \rho^{-O(t)}$ and  $|\B_c| = \rho_c^{-O(t)}$ where the constants in the exponent 
depends on $d$.
Observe that each shape in $\rho_{i,j_{j'}}$ is a subset of the top face of $\Q_i$, a $(d-1)$-dimensional region. 
Furthermore, for every shape $b \in \B$ we have $\vol_{(d-1)t}(b) = O(1)^t \rho$ and
for every shape $b \in \B_c$ we have $\vol_{(d-1)t}(b) = O(1)^t \rho_c$.

With these in mind, we now pick the set of parametric points.
We start with an initial placement and coloring:
for every color $c \in \C_g$, we create
a set containing $r/|\C_g|$  $t$-points  $\alpha_i^{(j)}$, $1 \le i \le r$, $1 \le j \le t$ of color $c$, where
the point $\alpha_i^{(j)}$ is placed randomly and uniformly on the top face of $\Q_j$. 
We now perform the following refinements.

\paragraph{Color Based Refinements.}
Consider a color $c \in \C_g$. 
If there exists $\beta$ sets $\S_1, \dots, \S_\beta$ with
color $c$, such that we have 
$\pvol(\S_1, \dots, \S_\beta) < 2^{-t}\rho_c$, then we remove one of those sets. 
By the end of the refinements, for the remaining sets, clearly we have
that $\pvol(\S_1, \dots, \S_\beta) \ge 2^{-t} \rho_c$.
We now estimate the expected number of sets that we remove in this refining step. 

Consider $\beta$ sets such that $\pvol(\S_1, \dots, \S_\beta) < 2^{-t}\rho_c$ with
$\phi(\S_i) = (\alpha_i^{(1)}, \dots, \alpha_i^{(t)})$.
Consider the convex hulls $R_j = \conv(\alpha_1^{(j)}, \alpha_2^{(j)}, \dots, \alpha_\beta^{(j)})$,
$1 \le j \le \beta$.
There exists an integer  $r_{j}$ such that 
$2^{-r_{j}-1} \le \vol_{d-1}(R_i)\le 2^{-r_{j}}$ which implies
$2^{-r_1 - r_2 - \dots - r_t} < \rho_c$.
Thus, by construction, there exists a region $R \in \B_c$ such that $\preg(\S_1, \dots, \S_\beta) \subset R$.
This implies to estimate the number of points removed in this refining step, it is simply sufficient to
estimate the expected number of points removed from each region $R \in \B_c$ and to add them up (using
the linearity of expectations).
Thus, consider a fixed region $R\in \B_c$.
We have that $\vol_{(d-1)t}(R) = O(1)^t \rho_c$.
We first calculate the probability of an event where we place more than $\beta$ points inside $R$.
Since the points of each 
The probability that we place a point inside $R$ is clearly exactly equal to $\vol_{(d-1)t}(R) = O(1)^t \rho_c$.
The probability that exactly $\beta'$ points are placed inside $R$ is upper bounded by
\[
    {r/|\C_g| \choose \beta'} O(1)^{t \beta'} \rho_c^{\beta'}.
\]
If $\beta' > \beta$, then we will remove some of the points placed in $R$.
In the worst case we might remove all of them which implies the expected number of points removed from 
$R$ is upper bounded by 
\[
    \sum_{\beta'> \beta}^\infty {r/|\C_g| \choose \beta'} O(1)^{t \beta'} \rho_c^{\beta'}\beta' = \sum_{\beta'> \beta}^\infty \Theta\left( \frac{r \rho_c}{|\C_g|\beta'} \right)^{\beta'} O(1)^{t \beta'} \beta' = \Theta\left( \frac{r \rho_c}{|\C_g|\beta} \right)^{\beta} 
\]
where we have used the assumption that $\rho_c = o( |\C_g| / (c_0^t r))$ for a constant $c_0$.

\paragraph{General Refinement.}
Finally, we perform another refinement similar to the point refinement. 
If there exists $\beta$ sets $\S_1, \dots, \S_\beta$ (possibly of different colors) such that 
$\pvol(\S_1, \dots, \S_\beta) < 2^{-t}\rho$, then we remove one of those sets. 
By the end of the refinements, for the remaining sets, clearly we have
that $\pvol(\S_1, \dots, \S_\beta) \ge 2^{-t} \rho$.
A very similar argument shows that the expected number of sets that we removed is bounded by 
\[
    \sum_{\beta'> \beta}^\infty {r \choose \beta'} O(1)^{t \beta'} \rho^{\beta'}\beta'= \Theta\left( \frac{r \rho}{\beta} \right)^{\beta} .
\]



We will pick $\rho, \rho_c$, and $\beta$ such that the expected number of sets removed will be bounded by a constant,
over all regions in $\B$ and $\B_c$, and thus we would like to bound
\begin{align}
    \rho_c^{-O(t)}  \Theta\left( \frac{r \rho_c}{|\C_g|\beta} \right)^{\beta} + \rho^{-O(t)} \Theta\left( \frac{r \rho}{\beta} \right)^{\beta} = O(1).
\end{align}
This will be the final construction. 
Note that we also have freedom in picking the parameters $\ell$, and $g$ that were used to prune the colors
(i.e., remember that $\C_g$ does not contain any $g$-bad $\ell$-subset). 


\paragraph{Analysing the volume of intersection.}
We now arrive at the main part of the analysis where we have to analyse the volume of the intersection
of a number of $t$-slabs.
Consider a set $\A$ of $\alpha$ $t$-slabs $\bs_1, \dots, \bs_\alpha$.
We consider the following cases.
\begin{itemize}
    \item Case 1: Two of the slabs in $\A$ are from the same set $\S_i$. 
        W.l.o.g, assume $\bs_1, \bs_2 \in \S_i$. 
        In this case, by construction, $\vol_{dt}(\bs_1 \cap \bs_2) = 0$ and thus all the $\alpha$ slabs have 0
        intersection volume. 
        Thus, in the remaining cases, we can assume 
        $\bs_i \in \S_i$ and $\S_i$'s are distinct. 
    \item Case 2: Consider the colors $\C(\S_1), \dots, \C(\S_\alpha)$.
        In this case, we assume there are at least $\sqrt{\alpha}$ identical colors among this set of colors. 
        Let $\alpha'= \sqrt{\alpha}$.
        W.l.o.g, assume $\C(\S_1) = \C(\S_2) = \dots = \C(\S_{\alpha'})$.
        By the color refinement, we know that if $\alpha' > \beta$, then
        $\pvol(\S_1, \dots, \S_{\alpha}) \ge 2^{-t}\rho_c$. 
        Thus, we will pick $\alpha$ such that $\sqrt{\alpha} > \beta$ and then
        we can find $d$ sets, w.l.o.g, assume $\S_1, \dots, \S_d$ such that
        $\pvol(\S_1, \dots, \S_{d}) \ge O(\alpha)^{-t}\rho_c$. 

        Thus, by Lemma~\ref{lem:parallel}, we have 
       \[
           \vol_{dt}(\bs_1 \cap \dots \bs_{d}) \le \prod_{j=1}^t\frac{\prod_{i=1}^{d}W_{i}^{(j)}}{\vol_{d-1}(\conv(\alpha_1^{(j)}, \alpha_2^{(j)}, \dots, \alpha_{d}^{(j)}))} \le \frac{\left( {n\over r} \right)^d}{O(\alpha)^{-t}\rho_c}.
       \]

   \item Case 3: Otherwise, there are at least $\alpha'= \sqrt{\alpha}$ sets that have distinct colors.
       W.l.o.g., assume all the colors $\C(\S_1), \C(\S_2), \dots, \C(\S_{\alpha'})$ are distinct. 
       In the rest of the proof and in the remaining cases, we only focus on the slabs $\bs_1, \dots, \bs_{\alpha'}$.
       Let $\A'$ be the set containing these slabs. 

       By construction, we know that the parametric volume of any $\beta$ slabs in $\A'$ is at least $\rho$.
       We claim this implies the existence of a subset $E$ of the these slabs that has size
       $\alpha'' = \Omega( \alpha'/\beta)^{1/d}$ such that the parametric volume of every $d$ slabs is
       at least $\rho/\alpha'$.
       To see this, let $E$ be a random subset of $\A'$ where each slab is sampled with probability
       $\varepsilon\alpha''/\alpha'$ for small enough constant $\varepsilon$. 
       The probability that $d$ randomly chosen slabs from $\A'$ form a volume smaller than $\rho$ is 
       at most 

       

\end{itemize}


\pagebreak

